SigVM: Enabling Event-Driven Execution for Autonomous Smart Contracts

This paper presents SigVM, a novel blockchain virtual machine that supports an event-driven execution model, enabling developers to build autonomous smart contracts. Contracts in SigVM can emit signal events, on which other contracts can listen. Once an event is triggered, corresponding handler functions are automatically executed as signal transactions. We build an end-to-end blockchain platform SigChain and a contract language compiler SigSolid to realize the potential of SigVM. Experimental results show that our benchmark applications can be reimplemented with SigVM in an autonomous way, eliminating the dependency on unreliable mechanisms like off-chain relay servers. The development effort of reimplementing these contracts with SigVM is small, i.e., we modified on average 2.6% of the contract code.

==> figures/blockexec.tex <==
% Process Execution Result
\begin{figure}[t]
\begin{minipage}{\columnwidth}
\begin{algorithm}[H]
\begin{algorithmic}
\Function{ProcessExec}{$\mathit{height}, \mathit{addr}, Q, A, M, L, E$}
    \State $Q' \gets Q$
    \ForAll{$\langle \mathit{addr} \circ a, S, l, \mathit{pc}, g \rangle \in E$}
        \State $\mathit{height'} \gets \mathit{height} + l + 1$
        \State $v \gets \langle \mathit{height'}, \mathit{addr}, \mathit{pc}, g, S \rangle$
        \State $Q' \gets Q'[\mathit{height'} \mapsto (Q[\mathit{height'}] \circ v)]$
    \EndFor
    \State \textbf{let} $\langle \_, \_, P \rangle = A(\mathit{addr})$
    \State \textbf{return} $\langle Q', A[\mathit{addr} \mapsto \langle M, L, P\rangle] \rangle$
\EndFunction
\caption{Process execution result}\label{algo:ProcessExec}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]

\begin{algorithmic}
\Function{ExecuteNewBlock}{$\sigma, B$}
%   \If{$\frac{\text{number of }SignalTx \text{ in }B}{\text{number of }Tx\text{ in }B} > \frac{1}{10}$} \\
%      \hspace{9mm} \textbf{return} 
%    \EndIf
    \For{$\text{every transaction }w\text{ in }B$}
        \State \textbf{suppose} $\sigma \llll \texttt{transact}(w) \rrrr^* \sigma'$
        \State $\sigma \gets \sigma'$
    \EndFor
    \State \textbf{let} $\langle \mathit{height}, R, Q, A, N \rangle = \sigma$
    \State $\mathit{height'} \gets \mathit{height} + 1$
    %\State $Q[\mathit{height} \mapsto \varnothing]$
    \ForAll{$v \in Q(\mathit{height'})$}
        \State \textbf{let} $\langle \_, \mathit{addr}, \_, \_, \_ \rangle = v$
        \State \textbf{let} $\langle M, L, P \rangle = A(\mathit{addr})$
        \State $A \gets A[\mathit{addr} \mapsto \langle M, L \circ v, P \rangle]$
    \EndFor
    \State \textbf{return} $\langle \mathit{height'}, R, Q[\mathit{height'} \mapsto \emptyset], A, N\rangle$
\EndFunction
\end{algorithmic}
\caption{Execute new block}\label{algo:ExecuteNewBlock}
\end{algorithm}
\end{minipage}
\end{figure}
% Block Creation
%\begin{algorithm}
%\begin{algorithmic}
%\Function{CreateNewBlock}{}
%        \State $B = \texttt{PackRegTx}() \circ \texttt{PackHandlerTx}()$
%    \State \textbf{return} $B$
%\EndFunction
%\end{algorithmic}
%\caption{Create new block}\label{algo:CreateNewBlock}
%\end{algorithm}


==> figures/implementation.tex <==
% Solidity Compiler Opcodes
\begin{figure}
\begin{tabular}{|l|l|}
\hline
\textbf{Opcode} & \textbf{Description} \\
\hline
\hline
\makecell{\texttt{createsignal}} & \makecell[l]{
    Create a signal on the blockchain state \\
    with the given signal key under the \\
    current call address \\.
    \begin{tabular}{l|l} 
        \textbf{Arg} & \textbf{Description} \\
        \hline
        0 & signal key \\
    \end{tabular} \\\\
} \\
\hline
\makecell{\texttt{deletesignal}} & \makecell[l]{
    Delete a signal \\
    \begin{tabular}{l|l} 
        \textbf{Arg} & \textbf{Description} \\
        \hline
        0 & signal key \\
    \end{tabular} \\\\
} \\
\hline
\makecell{\texttt{createhandler}} & \makecell[l]{
    Create a handler \\
    \begin{tabular}{l|l} 
        \textbf{Arg} & \textbf{Description} \\
        \hline
        0 & handler key \\
        1 & method hash \\
        2 & gas limit \\
        3 & gas ratio \\
    \end{tabular} \\\\
} \\
\hline
\makecell{\texttt{deletehandler}} & \makecell[l]{
    Delete a handler \\
    \begin{tabular}{l|l} 
        \textbf{Arg} & \textbf{Description} \\
        \hline
        0 & handler key \\
    \end{tabular} \\\\
} \\
\hline
\makecell{\texttt{sigemit}} & \makecell[l]{
    Emit a signal with data and delay \\
    \begin{tabular}{l|l} 
        \textbf{Arg} & \textbf{Description} \\
        \hline
        0 & signal key \\
        1 & data pointer \\
        2 & data length \\
        3 & delay \\
    \end{tabular} \\\\
} \\
\hline
\makecell{
    \texttt{sigbind}
} & \makecell[l]{
    Bind a handler to a signal \\
    \begin{tabular}{l|l} 
        \textbf{Arg} & \textbf{Description} \\
        \hline
        0 & handler key \\
        1 & signal contract address \\
        2 & signal prototype hash \\
    \end{tabular} \\\\
} \\
\hline
\makecell{\texttt{sigdetach}} & \makecell[l]{
    Detach a handler from a signal \\
    \begin{tabular}{l|l} 
        \textbf{Arg} & \textbf{Description} \\
        \hline
        0 & handler key \\
        1 & signal contract address \\
        2 & signal prototype hash \\
    \end{tabular} \\\\
} \\
\hline
\end{tabular}
\caption{Added Solidity Opcodes}\label{fig:implOpcodes}
\end{figure}

% Solidity Syntax Features
\begin{figure}
\begin{lstlisting}[language=Solidity, breaklines=true, numbers=none]
contract A {
    string foo;
    bytes32 bar;
    uint256 baz;
    signal  AlertSignal(string, bytes32, uint256);
    handler AlertHandle(string, bytes32, uint256);

    function Update(string memory fooo, bytes32 barr, uint256 bazz) public {
        foo = fooo;
        bar = barr;
        baz = bazz;
    }
    function Initialize() public {
        AlertSignal.create_signal();
        AlertHandle.create_handler(
            "Update(string,bytes32,uint256)", 
            10000, 
            120
        );
    }
    function Cleanup() public {
        AlertSignal.delete_signal();
        AlertHandle.delete_handler();
    }
    function Emit() public view {
        string memory foo = "foo is here";
        bytes32 bar = 0;
        uint baz = 2;
        AlertSignal.emit(foo, bar, baz).delay(5);
    }
    function Bind() public view {
        address this_address = address(this);
        AlertHandle.bind(
            this_address, 
            "AlertSignal(string,bytes32,uint256)"
        );
    }
    function Detach() public view {
        address this_address = address(this);
        AlertHandle.detach(
            this_address, 
            "AlertSignal(string,bytes32,uint256)"
        );
    }
}
\end{lstlisting}
\caption{Example Contract Before Parsing}\label{fig:implSyntax}
\end{figure}

% % Solidity Syntax
% \begin{figure}
% \begin{lstlisting}[language=C++, breaklines=true, numbers=none]
% contract A {
%     string foo;
%     bytes32 bar;
%     uint256 baz;
%     bytes32 private AlertSignal_key;
%     function set_AlertSignal_key() private {
%         AlertSignal_key = keccak256("AlertSignal(string,bytes32,uint256)");
%     }
%     // Original code: handler AlertHandle;
%     bytes32 private AlertHandle_key;
%     function set_AlertHandle_key() private {
%         AlertHandle_key = keccak256("AlertHandle(string,bytes32,uint256)");
%     }
%     function Update(string memory fooo, bytes32 barr, uint256 bazz) public {
%         foo = fooo;
%         bar = barr;
%         baz = bazz;
%     }
%     function Initialize() public {
%         // Original code: AlertSignal.create_signal();
%         set_AlertSignal_key();
%         assembly {
%             mstore(0x00, createsignal(sload(AlertSignal_key.slot)))
%         }
%         set_AlertHandle_key();
%         bytes32 AlertHandle_method_hash = 
%             keccak256("Update(string,bytes32,uint256)");
%         uint AlertHandle_gas_limit = 10000;
%         uint AlertHandle_gas_ratio = 120;
%         assembly {
%             mstore(
%                 0x00, 
%                 createhandler(
%                     sload(AlertHandle_key.slot), 
%                     AlertHandle_method_hash, 
%                     AlertHandle_gas_limit, 
%                     AlertHandle_gas_ratio
%                 )
%             )
%         }
%     }
%     function Cleanup() public {
%         AlertSignal_key = 0;
%         assembly {
%             mstore(0x00, deletesignal(sload(AlertSignal_key.slot)))
%         }
%         AlertHandle_key = 0;
%         assembly {
%             mstore(0x00, deletehandler(sload(AlertHandle_key.slot)))
%         }
%     }
%     function Emit() public view {
%         string memory foo = "foo is here";
%         bytes32 bar = 0;
%         uint baz = 2;
%         bytes memory abi_encoded_AlertSignal_data = abi.encode(foo,bar,baz);
%         uint abi_encoded_AlertSignal_length = abi_encoded_AlertSignal_data.length;
%         assembly {
%             mstore(
%                 0x00,
%                 sigemit(
%                     sload(AlertSignal_key.slot), 
%                     abi_encoded_AlertSignal_data,
%                     abi_encoded_AlertSignal_length,
%                     5
%                 )
%             )
%         }
%     }
%     function Bind() public view {
%         address this_address = address(this);
%         bytes32 AlertHandle_signal_prototype_hash = 
%             keccak256("AlertSignal(string,bytes32,uint256)");
%         assembly {
%             mstore(
%                 0x00,
%                 sigbind(
%                     sload(AlertHandle_key.slot),
%                     this_address,
%                     AlertHandle_signal_prototype_hash
%                 )
%             )
%         }
%     }
%     function Detach() public view {
%         address this_address = address(this);
%         bytes32 AlertHandle_signal_prototype_hash = 
%             keccak256("AlertSignal(string,bytes32,uint256)");
%         assembly {
%             mstore(
%                 0x00,
%                 sigdetach(
%                     sload(AlertHandle_key.slot),
%                     this_address,
%                     AlertHandle_signal_prototype_hash
%                 )
%             )
%         }
%     }
% }  
% \end{lstlisting}
% \caption{Example Contract After Parsing}\label{fig:implSyntaxParsed}
% \end{figure}

==> figures/syntax.tex <==
% Machine State
\begin{figure}
\centering
\begin{align*}
    I &\in Inst ::= \ \texttt{pop}\  |\ \texttt{push} \ a\ |\ \texttt{dup}\ |\ \texttt{swap}\ \\
        &\ \ \ \ |\ \texttt{load} \ |\ \texttt{store} \ |\ \texttt{add}\ |\ \texttt{jump}\ |\ \texttt{stop}  \\ 
        &\ \ \ \ |\ \texttt{createsignal}\  |\ \texttt{deletesignal}\ \\
        &\ \ \ \ |\ \texttt{emit}\  | \ \texttt{bind}\  |\ \texttt{detach}\ \\
    P &\in Program ::= \mathit{pc} \mapsto I \\
    \mu &\in ExecEnvironment ::= \langle \mathit{pc}, G, \mathit{gas},\mathit{addr},S,M,R,E\rangle \\
    S &\in Stack ::= x_1 \circ x_2 \circ \ldots \circ x_n \\
    M &\in StorageMap ::= a \mapsto x \\
    R &\in SignalRecordMap ::= k \mapsto H \\
    k &\in Key ::= \langle \mathit{addr}, a \rangle\\
    H &\in HandlerRecordSet ::= \{h_1, h_2, \ldots\} \\
    h_i &\in HandlerRecord ::= \langle \mathit{addr}, \mathit{pc}, g\rangle \\
    E &\in EmitSignalSet ::= \{e_1, e_2, \ldots\} \\
    e_i &\in EmitSignalRecord ::= \langle  k, S, l, \mathit{pc}, g\rangle \\
\end{align*}
\begin{displaymath}
    \mathit{addr}, G, \mathit{pc}, \mathit{gas}, a, b, y, z, g, l, x_i \in \mathbb{N}_{32}
\end{displaymath}
\caption{Core Language Syntax of {\name}}\label{fig:languageSyntax}
\end{figure}
% Block Chain State
\begin{figure}
\centering
\begin{align*}
    B &\in Block ::= \langle \mathit{height}, T, U, V \rangle \\
    T &\in CreateTxSet :: \{ t_1, t_2, \ldots \} \\
    t_i &\in CreateTx ::= \langle \mathit{addr}, s, n, b, C \rangle \\
    U &\in RegularTxSet ::= \{ u_1, u_2, \ldots \} \\
    u_i &\in RegularTx ::= \langle s, \mathit{addr}, n, b, \mathit{pc}, S\rangle \\
    V &\in SignalTxSet ::= \{ v_1, v_2, \ldots \} \\
    v_i &\in SignalTx ::= \langle \mathit{height}, \mathit{addr}, \mathit{pc}, g, S \rangle \\
    \sigma &\in BlockchainState ::= \langle \mathit{height}, B, R, Q, A, N\rangle \\	
    Q &\in TxQueueMap ::= \mathit{height} \mapsto L \\ 
    L &\in TxQueue ::= v_1 \circ v_2 \ldots \circ v_n \\
    A &\in AccountStateMap ::= \mathit{addr} \mapsto D \\
    D &\in StateRecord ::= \langle M, L, P \rangle \\
    N &\in AccountNonceMap ::= \mathit{addr} \mapsto F \\
    F &\in BalanceRecord ::= \langle n, b \rangle \\    
\end{align*}
\begin{displaymath}
    \mathit{height}, s, n \in \mathbb{N}_{32}
\end{displaymath}
\caption{Block, Transaction, and Blockchain State Syntax}\label{fig:stateSyntax}
\end{figure}

